Uncertainty-Aware Budget Allocation for Adaptive Test-Time Reasoning

Sampling multiple responses improves language model reasoning, but uniform compute allocation is inefficient because easy questions are over-sampled while hard questions remain under-explored. We propose \textbf{Uncertainty-Aware Budget Allocation (UAB)}, a concave integer optimization framework that reallocates a fixed sampling budget using uncertainty estimated from the initial samples themselves. In Phase-1, every question receives a small fixed number of generations. Their answer disagreement, measured by vote entropy, provides a difficulty signal while these generations contribute to the final vote. In Phase-2, the remaining budget is allocated by a marginal-greedy algorithm that optimally solves a concave coverage-maximization surrogate, concentrating samples on questions whose initial answers disagree. Across five open-weight models (1.5B--27B parameters) and five reasoning benchmarks of varying difficulty, UAB improves average accuracy by $+2.3\%$ over uniform allocation, and achieves gains of up to $+5.5\%$ on individual benchmarks, with the largest gains in low-resource settings. Moreover, UAB meets the target budget exactly and requires no auxiliary model or additional LLM calls. Code is publicly available at https://github.com/manhitv/UAB.

==> tables/review_oracle_stable.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt}
\caption{Oracle($q$) under two definitions. \textit{First} is the smallest sample prefix whose majority vote is correct, which the main text uses, while \textit{Stable} additionally requires the vote to stay correct for every larger prefix up to $16$ samples, so a lucky prefix does not count. \%Censored is the share of questions for which the definition is never satisfied within $16$ samples and which are therefore excluded.}
\label{tab:oracle_stable}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\textbf{Model} & \textbf{Dataset} & \textbf{First} & \textbf{Stable} & \textbf{\%Censored (first)} & \textbf{\%Censored (stable)} \\
\midrule
\multirow{5}{*}{Qwen2.5-1.5B} & MATH500 & 2.36 & 3.11 & 40.1 & 46.6 \\
 & Formal Logic & 1.59 & 2.05 & 46.8 & 56.6 \\
 & DeepScaler & 2.91 & 4.68 & 69.3 & 76.3 \\
 & GSM8K & 2.45 & 4.07 & 16.6 & 24.6 \\
 & Graded Arith. & 2.27 & 3.17 & 31.7 & 36.3 \\
\midrule
\multirow{5}{*}{Llama3.2-3B} & MATH500 & 3.23 & 4.20 & 49.1 & 56.2 \\
 & Formal Logic & 2.74 & 4.46 & 34.1 & 55.8 \\
 & DeepScaler & 2.47 & 4.09 & 74.8 & 80.4 \\
 & GSM8K & 1.67 & 2.55 & 12.9 & 17.6 \\
 & Graded Arith. & 1.41 & 1.61 & 33.0 & 37.0 \\
\midrule
\multirow{5}{*}{Qwen2.5-7B} & MATH500 & 1.51 & 1.97 & 27.7 & 32.1 \\
 & Formal Logic & 1.72 & 2.40 & 27.0 & 36.5 \\
 & DeepScaler & 2.75 & 4.03 & 56.1 & 68.2 \\
 & GSM8K & 1.45 & 1.80 & 4.3 & 6.1 \\
 & Graded Arith. & 1.90 & 2.97 & 26.0 & 30.0 \\
\bottomrule
\end{tabular}
}
\end{table}

